CultureVLM: Characterizing and Improving Cultural Understanding of Vision-Language Models for over 100 Countries

Vision-language models (VLMs) have advanced human-AI interaction but struggle with cultural understanding, often misinterpreting symbols, gestures, and artifacts due to biases in predominantly Western-centric training data. In this paper, we construct CultureVerse, a large-scale multimodal benchmark covering 19, 682 cultural concepts, 188 countries/regions, 15 cultural concepts, and 3 question types, with the aim of characterizing and improving VLMs' multicultural understanding capabilities. Then, we propose CultureVLM, a series of VLMs fine-tuned on our dataset to achieve significant performance improvement in cultural understanding. Our evaluation of 16 models reveals significant disparities, with a stronger performance in Western concepts and weaker results in African and Asian contexts. Fine-tuning on our CultureVerse enhances cultural perception, demonstrating cross-cultural, cross-continent, and cross-dataset generalization without sacrificing performance on models' general VLM benchmarks. We further present insights on cultural generalization and forgetting. We hope that this work could lay the foundation for more equitable and culturally aware multimodal AI systems.

==> table/concept_category.tex <==
% 
% \begin{table*}[htbp]
%     \centering
%     \resizebox{.9\textwidth}{!}{
%     \begin{tabular}{lll}  
%         \toprule  
%         \textbf{Category} & \textbf{Sub Category} & \textbf{Example Description} \\  
%         \midrule  
%         Natural Environment and Local Resources & Food & Local specialty dishes, traditional festival foods \\  
%         Natural Environment and Local Resources & Plants & Unique flowers, crops in a certain area \\  
%         Natural Environment and Local Resources & Animals & Unique wild animals, livestock in a certain area \\ 
%         History and Landmarks & Famous Landmarks & Famous historical sites, buildings \\  
%         Cultural Heritage and Traditions & Festivals & Unique festival celebration scenes \\  
%         History and Landmarks & Historical Artifacts & Museum collections, ancient relics \\  
%         History and Landmarks & Historical Figures & Portraits of historical figures, statues \\  
%         Cultural Heritage and Traditions & Traditional Clothing & Ethnic clothing, festival attire \\  
%         History and Landmarks & Architectural Styles & Traditional architecture, modern landmark buildings \\  
%         Cultural Heritage and Traditions & Handicrafts and Artifacts & Ethnic handicrafts, traditional handmade items \\  
%         Cultural Heritage and Traditions & Music and Dance & Traditional musical instruments, dance scenes \\  
%         Cultural Heritage and Traditions & Religion and Belief & Temples and churches, religious ceremonies \\  
%         Natural Environment and Local Resources & Natural Scenery and Ecosystems & Unique natural landscapes, ecological reserves \\  
%         Natural Environment and Local Resources & Markets and Shopping Traditions & Local markets, specialty shops \\  
%         Cultural Heritage and Traditions & Entertainment and Performing Arts & Theater performances, street performers \\  
%         \bottomrule  
%     \end{tabular}  
%     }
%     \caption{Collected concepts, their main categories, and descriptions in the dataset.}
%     \label{tb-concept-category}
% \end{table*}




